Multi-Object Reasoning with Constrained Goal Models

Goal models have been widely used in Computer Science to represent software requirements, business objectives, and design qualities. Existing goal modelling techniques, however, have shown limitations of expressiveness and/or tractability in coping with complex real-world problems. In this work, we exploit advances in automated reasoning technologies, notably Satisfiability and Optimization Modulo Theories (SMT/OMT), and we propose and formalize: (i) an extended modelling language for goals, namely the Constrained Goal Model (CGM), which makes explicit the notion of goal refinement and of domain assumption, allows for expressing preferences between goals and refinements, and allows for associating numerical attributes to goals and refinements for defining constraints and optimization goals over multiple objective functions, refinements and their numerical attributes; (ii) a novel set of automated reasoning functionalities over CGMs, allowing for automatically generating suitable refinements of input CGMs, under user-specified assumptions and constraints, that also maximize preferences and optimize given objective functions. We have implemented these modelling and reasoning functionalities in a tool, named CGM-Tool, using the OMT solver OptiMathSAT as automated reasoning backend. Moreover, we have conducted an experimental evaluation on large CGMs to support the claim that our proposal scales well for goal models with thousands of elements.

==> evolving_goalmodels_functionalities.tex <==
%\RSTODO{Explain}

%
  
Proposition~\ref{prop:main_evolving} suggests that, when modifying 
a WCGM $\calm_1$ having a realization $\mu_1$ 
into a new one $\calm_2$, the realization $\mu_2$ which minimizes 
the primitive goals to be satisfied from scratch can be 
encoded into a OMT problem. 
%
This allows for  implementing straightforwardly the following reasoning
functionality on WCGMs, in addition to those described in
\sref{sec:goalmodels_functionalities} and
\sref{sec:weighted_goalmodels_functionalities}.  
 

\begin{description}

\item[Search/enumerate minimum-penalty WCGM realizations.] 
Given a WCGM $\calm_2$ and a realization $\mu_1$ of a previous version 
of  $\calm_2$, 
 it is
  possible to find one (many, all)  realization(s) which
  achieve the desired assertions while minimizing the total penalty of 
  priced leaf goals which are either new in $\calm_2$ or were not 
previously realized in $\mu_1$.
%
This is achieved by choosing the assertions $\assertions$ and by
 setting the penalties of all priced leaf goals and then running the OMT
 solver on the OMT problem \tuple{\encaddcostass,\cost}. 


\end{description}




==> extrachart.tex <==
\begin{figure*}
\centering 
\includegraphics[height=0.95\textheight]{MediaRunTimeComp_cost.pdf}
\caption{Experimental Median Runtime Comparision: Cost Optimization}
\label{figGMEx}
\end{figure*}

\begin{figure*}
\centering 
\includegraphics[height=0.95\textheight]{MediaRunTimeComp_time.pdf}
\caption{Experimental Median Runtime Comparision: Time Optimization}
\label{figGMEx}
\end{figure*}

\begin{figure*}
\centering 
\includegraphics[height=0.95\textheight]{MediaRunTimeComp_weight.pdf}
\caption{Experimental Median Runtime Comparision: Weight Optimization}
\label{figGMEx}
\end{figure*}

\begin{figure*}
\centering 
\includegraphics[height=0.95\textheight]{MediaRunTimeComp_ctw.pdf}
\caption{Experimental Median Runtime Comparision: Cost/Time/Weight Lex-Order Optimization}
\label{figGMEx}
\end{figure*}

\begin{figure*}
\centering 
\includegraphics[height=0.95\textheight]{MediaRunTimeComp_wtc.pdf}
\caption{Experimental Median Runtime Comparision: Weight/Time/Cost Lex-Order Optimization}
\label{figGMEx}
\end{figure*}



==> goalmodels_sugar.tex <==



In general, the user may not be at ease in defining
a %possibly-complex
global propositional formula $\Psi$ to encode constraints among goals
and refinements.  To this extent, as 
syntactic sugar, it is easy to provide some extra constructs allowing the
user to encode {\em easily} and {\em locally} some desired constraints. 

First, it is easy to provide the user the possibility of
performing the following actions.

\begin{enumerate}
\item  Draw some other kind of 
edges of common usage, in particular: 
%
\begin{description}
\item[Element-contribution edges,] denoted as
  $\contributes{E_1}{E_2}$, meaning that 
satisfying $E_1$ forces $E_2$ to be satisfied (but not vice versa). 
(The edge
$\bicontributes{E_1}{E_2}$ can be used to merge the
two contribution edges
$\contributes{E_1}{E_2}$ and
$\contributes{E_2}{E_1}$ into one.)
 This is implemented by adding  to $\Psi$ the formula $(E_1\imp
 E_2)$. 
\item[Element-conflict edges,] denoted as
  $\conflict{E_1}{E_2}$, meaning that 
$E_1$ and $E_2$ cannot be
  satisfied simultaneously. 
 This is implemented by adding  to $\Psi$ the formula
$(\neg E_1\vee\neg E_2)$.
%
\item[Refinement-binding edges,]  denoted as 
%$R_1 \leftarrow -  \rightarrow R_2$ 
  $\bind{\Refinement{R_1}}{\Refinement{R_2}}$, meaning that, if both 
the target goals of $R_1$ and $R_2$ (namely $G_1$ and  $G_2$
respectively) are satisfied, then $R_1$ refines $G_1$  if and only if 
$R_2$ refines $G_2$.
 This is implemented by adding  to $\Psi$ the formula
$$
(G_1 \wedge G_2) 
\imp 
(\Refinement{R_1}\iff\Refinement{R_2}).
$$
%

\item[Preference edge,] denoted as $\preferred{A_1}{A_2}$, meaning that we
would want to have the element or refinement $A_1$ to be satisfied (and do not care about $A_2$)
instead of the case where the element or refinement $A_2$ satisfied while $A_1$ is not.
Note that this does not have any constraint over the case where $A_1$ and $A_2$ 
are both satisfied or both unsatisfied at the same time.
This is implemented by adding to $\Psi$ the formula below as soft constraint:
$$
(A_1 \vee (\neg A_2))
$$
Note that: $A_1$ and $A_2$ should be of the same kind, i.e. both are either tasks, requirements, refinements, intermediate goals, or domain assumptions.


\end{description}
% 
\noindent
Notice that element-contribution, element-conflict and refinement-binding
edges are allowed to form loops.
%

\item Add ``local'' pre-requisite constraints to goal
  nodes $G_i$  or to refinements $R_j$. 

\begin{description}
  \item[Goal prerequisite constraints:]
for each goal $\Goal{G}$ it is possible to introduce locally  a pair 
of propositional constraints $\Constraint{G}{\phi}$ on \calb, so that 
 $\posConstraint{G}{\phi}$ (resp. $\negConstraint{G}{\phi}$) must be
 satisfied whenever the goal $\Goal{G}$ is  
satisfied (resp. denied), but not vice versa.
 This is implemented by adding  to $\Psi$ the formulas
$(G\imp \posConstraint{G}{\phi})$ 
and
$(\neg G\imp \negConstraint{G}{\phi})$ respectively.

  \item[Refinement prerequisite constraints:] same as with goals.
\RSNOTE{are they of actual use?}
\end{description}

{\item Force [unforce]  interactively element $E_i$ to be satisfied or
  denied.~%
\footnote{Typically the user may try to force root element to be
  satisfied, to achieve 
  a desired result, and/or to force leaf element to be denied, to reduce the effort.}
 This is implemented by adding to [dropping from] $\assertions{}$ 
the truth value assignments $(E_i)$ or $(\neg E_i)$ respectively.}


\ignore{
   A CGM augmented with contribution and conflict edges is easily
   converted into a plain CGM by removing them and adding to $\Psi$ the
   corresponding constraints in the form $(E_1\imp E_2)$ and $\neg
   (E_1\wedge E_2)$ respectively.
}

\item Force [unforce]  interactively refinements $R_j$ to be satisfied or
  denied. 
 This is implemented by adding to [dropping from] $\assertions{}$ 
the truth value assignments $(R_j)$ or $(\neg R_j)$ respectively.

\end{enumerate}


Second, is is easy to provide the user the possibility of defining, both
globally and locally, the most
standard and intuitive 
constraints among assumption, goal and refinement labels,
 with no need of defining
the corresponding complicate or less-intuitive propositional formulas. 
(In what follows, $P_1,...,P_i$ denote atomic propositions in \calb.)

\begin{itemize}
\item[$\predicate{Alt}{P_1,P_2}$] denotes the fact
$P_1$ and $P_2$ are alternative, e.g., that one and only one of them 
is satisfied. 
This can
  be encoded by the formula $(P_1\iff \neg P_2)$. 
\item[$\predicate{Causes}{P_1,P_2}$] denotes the fact
  that satisfying $\Goal{P_1}$  causes $\Goal{P_2}$ to be satisfied.
This can
  be encoded by the formula $(P_1\imp P_2)$. 
\item[$\predicate{Requires}{P_1,P_2}$] denotes the fact
  that satisfying $\Goal{P_1}$ requires $\Goal{P_2}$ to be satisfied.
This can be encoded by the formula $(P_1\imp P_2)$. 

\item[$\predicate{AtMostOneOf}{\{P_1,...,P_n\}}$] denotes the fact that at most
  one of $\{P_1,...,P_n\}$ must be satisfied. This can be  encoded 
by the formula  $\bigl(\bigwedge_{1 \leq i < j \leq n} (\neg P_i \vee
\neg P_j)\bigr)$.  

\item[$\predicate{AtLeastOneOf}{\{P_1,...,P_n\}}$] denotes the fact
  that at least one of $\{P_1,...,P_n\}$ must be satisfied. This can
  be encoded by the formula $\bigl(\bigvee_{1 \leq i \leq n}
  P_i\bigr)$.
\item[$\predicate{OneOf}{\{P_1,...,P_n\}}$] denotes the fact
  that exactly one of $\{P_1,...,P_n\}$ must be satisfied. This can
  be encoded by the conjunction of the latter two formulas.

\item[$\predicate{AtMostN}{N,\{P_1,...,P_n\}}$] denotes the fact that at most
  one of $\{P_1,...,P_n\}$ must be satisfied. This can be  encoded 
by Boolean cardinality constraints (see, e.g., \cite{RM09HBSAT}).
~\footnote{
Since the propositional encodings of these constraints is much more
complicate, we refer the reader to the wide literature on SAT
encodings of cardinality
constraints, in particular to \cite{RM09HBSAT} as a starting point.  
}  

\item[$\predicate{AtLeastN}{N,\{P_1,...,P_n\}}$] denotes the fact
  that at least one of $\{P_1,...,P_n\}$ must be satisfied. This can
  be encoded by  Boolean cardinality constraints.
\item[$\predicate{ExactlyN}{N,\{P_1,...,P_n\}}$] denotes the fact
  that exactly one of $\{P_1,...,P_n\}$ must be satisfied. This can
  be encoded by  Boolean cardinality constraints.

%\RSTODO{add atmost(N,...),atleast(N,...) Exactly(N,...)}

\end{itemize}

\RSTODO{Add syntactic sugaring for ``sourceOf'', ``targetOf'',
  ``refinementOf''.
Add  syntactic sugaring for multiple instantiations ``foreach'' 
(similar to bash ``for'' command).}


==> rs_macros_colors.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% cambiate in modo da gestire le animazioni
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \newcommand{\blue}[1]{\textcolor{blue}{#1}}
% \newcommand{\darkblue}[1]{\textcolor{blue}{#1}}
% \newcommand{\lightblue}[1]{\textcolor{lightblue4}{#1}}
% \newcommand{\red}[1]{\textcolor{red}{#1}}
% \newcommand{\green}[1]{\textcolor{darkgreen}{#1}}
% \newcommand{\lightgreen}[1]{\textcolor{palegreen1}{#1}}
% \newcommand{\violet}[1]{\textcolor{violet}{#1}}
% \newcommand{\darkviolet}[1]{\textcolor{darkviolet}{#1}}
% \newcommand{\darkgrey}[1]{\textcolor{darkgrey}{#1}}
% \newcommand{\palegrey}[1]{\textcolor{lightgrey}{#1}}
% \newcommand{\gray}[1]{\textcolor{gray}{#1}}
% \newcommand{\white}[1]{\textcolor{white}{#1}}
% \newcommand{\black}[1]{\textcolor{black}{#1}}
% \newcommand{\orange}[1]{\textcolor{orange}{#1}}
% \newcommand{\darkorange}[1]{\textcolor{darkorange3}{#1}}
%\newcommand<>{\orange}{\color#1{orange}}

\newcommand<>{\blue}{\color#1{blue}}
\newcommand<>{\darkblue}{\color#1{blue}}
\newcommand<>{\lightblue}{\color#1{lightblue4}}
\newcommand<>{\red}{\color#1{red}}
\newcommand<>{\green}{\color#1{darkgreen}}
\newcommand<>{\lightgreen}{\color#1{palegreen1}}
\newcommand<>{\violet}{\color#1{violet}}
\newcommand<>{\darkviolet}{\color#1{darkviolet}}
\newcommand<>{\darkgrey}{\color#1{darkgrey}}
\newcommand<>{\palegrey}{\color#1{lightgrey}}
\newcommand<>{\gray}{\color#1{gray}}
\newcommand<>{\white}{\color#1{white}}
\newcommand<>{\black}{\color#1{black}}
\newcommand<>{\orange}{\color#1{orange}}
\newcommand<>{\darkorange}{\color#1{darkorange3}}


==> rs_macros_dl.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% This file is an hard link, whose source is in   
%%%%%%% cipeciop.science.unitn.it:/home/rseba/latex/macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\en}[2]{{#1}e{#2}}
\newcommand{\den}[4]{\en{#1}{#2}/\en{#3}{#4}}

\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\msf}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\snomed}{\textsc{Snomed-CT}\xspace}
\newcommand{\geneonto}{\textsc{GeneOntology}\xspace}
\newcommand{\nci}{\textsc{NCI}\xspace}
\newcommand{\galen}{\textsc{Galen}\xspace}

\newcommand{\shsnomed}{\textsc{Snomed09}\xspace} 
\newcommand{\shnci}{\textsc{NCI}\xspace} 
\newcommand{\shgalen}{\textsc{notGalen}\xspace}
\newcommand{\shfullgalen}{{\textsc{fullGalen}}\xspace}
\newcommand{\shgeneontology}{{\textsc{GeneOnt.}}\xspace}

\newcommand{\conj}{\sqcap}
\newcommand{\disj}{\sqcup}
\newcommand{\exr}[2]{{\exists}#1.#2}

\newcommand{\subs}{\sqsubseteq}
\newcommand{\sups}{\sqsupseteq}
\newcommand{\norm}{\triangleq}
\newcommand{\comp}{\circ}

\newcommand{\topt}{\ensuremath{\top}\xspace}
\newcommand{\bott}{\ensuremath{\bot}\xspace}
\newcommand{\conjt}[2]{\ensuremath{#1 \sqcap #2}\xspace}
\newcommand{\disjt}[2]{\ensuremath{#1 \sqcup #2}\xspace}
\newcommand{\exrt}[2]{\ensuremath{{\exists}#1.#2}\xspace}
\newcommand{\equivt}[2]{\ensuremath{#1 \equiv #2}\xspace}
\newcommand{\subst}[2]{\ensuremath{#1 \sqsubseteq #2}\xspace}
\newcommand{\supst}[2]{\ensuremath{#1 \sqsupseteq #2}\xspace}
%\newcommand{\eqdef}{\stackrel{def}{=}}
%\newcommand{\defas}{\ensuremath{\stackrel{\text{\tiny def}}{=}}\xspace}
 
\newcommand{\pr}[1]{\ensuremath{p_{#1}}\xspace}
\newcommand{\prc}[1]{\ensuremath{p_{[#1]}}\xspace}
\newcommand{\sel}[1]{\ensuremath{s_{#1}}\xspace}
\newcommand{\selc}[1]{\ensuremath{s_{[#1]}}\xspace}

\newcommand{\goal}{\ensuremath{C_i\subs_\T D_i}\xspace}
\newcommand{\goalsure}{\ensuremath{C_i~\subs_\T~D_i}\xspace}
\newcommand{\tgoal}[1]{\ensuremath{C_i\subs_{#1} D_i}\xspace}
\newcommand{\igoal}[1]{\ensuremath{{C_{#1} \subs_\T D_{#1}}}\xspace}
\newcommand{\sgoal}{\ensuremath{\selc{\goal}}\xspace}
\newcommand{\isgoal}[1]{\ensuremath{\selc{\igoal{#1}}}\xspace}
\newcommand{\nsgoal}{\ensuremath{\neg\selc{C_i\subs_\T D_i}}\xspace}

\newcommand{\assumptiongoal}{\ensuremath{\{\neg\prc{D_i},\prc{C_i}\}}\xspace}
\newcommand{\assumptionsgoal}{\ensuremath{\{\neg\sgoal\}}\xspace}

\newcommand{\aenc}[1]{\ensuremath{\elp2sat(#1)}\xspace}
\newcommand{\wffsubs}{\ensuremath{\phi_{\T{}}}\xspace}
\newcommand{\wffsubsnotrans}{\ensuremath{\phi_{\T{}}^{notrans}}\xspace}
\newcommand{\wffmina}{\ensuremath{\wffsubs^{one}}\xspace}
\newcommand{\wffminarule}{\ensuremath{\phi_{\T(po)}^{one}}\xspace}
\newcommand{\wffminaT}[1]{\ensuremath{\phi_{#1}^{one}}\xspace}
\newcommand{\wffminaTrule}[1]{\ensuremath{\phi_{#1}^{one}}\xspace}
\newcommand{\wffallmina}{\ensuremath{\wffsubs^{all}}\xspace}
\newcommand{\wffallminarule}{\ensuremath{\phi_{\T{}(po)}^{all}}\xspace}
\newcommand{\wffallminaT}[1]{\ensuremath{\phi_{#1}^{all}}\xspace}
\newcommand{\wffallminaTrule}[1]{\ensuremath{\phi_{#1 (po)}^{all}}\xspace}
\newcommand{\wffallminaO}{\ensuremath{\phi_{\T^*}^{all}}\xspace}
\newcommand{\wffallminaruleO}{\ensuremath{\phi_{\T^*(po)}^{all}}\xspace}

\newcommand{\pinpointingwff}{\ensuremath{\Phi^{\goal}}\xspace}
\newcommand{\pinpointingwffall}{\ensuremath{\Phi^{all}}\xspace}

\newcommand{\hatT}{\ensuremath{\hat{\T}}\xspace}
\newcommand{\Tp}{\ensuremath{\ensuremath{\mathcal{T'}}\xspace}}

\newcommand{\elsat}{{\elp{}\textsc{SAT}}\xspace}















\newcommand{\el}{\ensuremath{\mathcal{EL}}\xspace}
\newcommand{\elh}{\ensuremath{\mathcal{ELH}}\xspace}
\newcommand{\elp}{\ensuremath{\mathcal{EL^{+}}}\xspace}
\newcommand{\elpp}{\ensuremath{\mathcal{EL^{++}}}\xspace}
\newcommand{\eloh}{\ensuremath{\mathcal{ELOH}}\xspace}
\newcommand{\eqdef}{\stackrel{def}{=}}


% \newcommand{\sel}[1]{\ensuremath{s_{#1}}\xspace}
% \newcommand{\selc}[1]{\ensuremath{s_{[#1]}}\xspace}
% \newcommand{\sgoal}{\ensuremath{\selc{\goal}}\xspace}
% \newcommand{\isgoal}[1]{\ensuremath{\selc{\igoal{#1}}}\xspace}
% \newcommand{\nsgoal}{\ensuremath{\neg\selc{C_i\subs_\T D_i}}\xspace}
% \newcommand{\aenc}[1]{\ensuremath{\elp2sat(#1)}\xspace}
% \newcommand{\elsat}{{\elp{}\textsc{SAT}}\xspace}






 


==> weighted_goalmodels.tex <==
%% DONE (RS)
%\RSTODO{Convert everything from MaxSAT to Pseudo-Boolean constraints
%or OMT?}



==> weighted_goalmodels_structure.tex <==
\begin{definition}[Weighted CGM]
\label{def:wcgm}
%\RSNOTE{What is the sense of having penalties with domain assumptions?\\}
%
A \new{Weighted Constrained Goal Model (WCGM)} is a tuple
\tuple{\calb,\caln,\cald,\Psi,\calw}, s.t. 
\tuple{\calb,\caln, \cald, \Psi} is a CGM 
% are as in Definition~\ref{def:cgm}, 
and 
$\calw:\calg\longmapsto \mathbb{Q}%\cup\{-\infty,+\infty\}
$ 
is a function which assigns  to each element 
$E_i\in\cale$ a rational number,~%
% \footnote{%
% The usage of integer values here is not mandatory, 
% and derives from the fact that 
% we use MaxSAT solvers as backend engines, which require integer-valued
% weights. 
% We could have rational-valued weights if we used
% instead an Optimization Modulo Theory solver \cite{sebastiani15_optimathsat}.
% } 
such that: 
\begin{itemize}
\item $\calw(E_i)\ge 0$ if $E_i$ is a leaf element {(task or
    assumption)},
\item $\calw(E_i)=   0$ if $E_i$ is an intermediate element,
\item $\calw(E_i)\le 0$ if $E_i$ is a root goal {(requirement)}.
\end{itemize}
%
\end{definition}
%
We call $\calw(E_i)$ the \new{weight} of $E_i$;
if $\calw(E_i)$ is strictly positive, we also call it 
the \new{penalty} of the (leaf) element $E_i$;
if it is strictly negative, we call $-\calw(E_i)$ the
\new{reward} of the requirement $E_i$.
%
\noindent
%Notationally, we often write $\calw(E_i)$ for $\calw(E_i)$.
%
When  $\calw(E_i)$ is not specified, we assume by default 
$\calw(E_i)= 0$. 


\begin{definition}[Realization, weight  of a realization and minimum weight of a
  WCGM.] 
%
  Let $\calm\defas\tuple{\calb,\caln,\cald,\Psi,\calw}$ be a WCGM.
% , and let
% \assertions{} be a set of user assertions defined as in Definition~\ref{def:realization}. 
%
  A \new{realization} $\mu$ of 
%  \tuple{\calm,\assertions} of 
\calm is a realization of \calm', 
%  \tuple{\calm',\assertions}. 
s.t. $\calm'\defas \tuple{\calb,\caln,\cald,\Psi}$
  is the un-weighted 
  version of \calm.  
%
We call the \new{weight} of $\mu$,
  denoted as \weightof{\mu}, the value
  \begin{eqnarray}
\label{eq:realizationweight}
%\ignoreinlong{\textstyle}
%\textstyle
    \sum_{E_i\in\cale,\mu(E_i)=\top} \calw(E_i).
  \end{eqnarray}
We call the \new{minimum weight} of \calm,
%\tuple{\calm,\assertions}, 
denoted as
\minweightof{\calm}, the value:
  \begin{eqnarray}
%\ignoreinlong{\textstyle}
min_{\{\mu\ realization\ of\ \calm\}}  \weightof{\mu}.
  \end{eqnarray}
\label{def:weightrealization}
\end{definition}  



\noindent
Notice that  \eqref{eq:realizationweight} is the difference between the
total penalties of leaf elements  and the total rewards 
of the requirements which are satisfied in the realization. 
Notice also that, if $E_i$ is a user assertion, then its truth value is
forced in every realization by a unit clause inside $\Psi$,
s.t. its weight plays no role in finding a minimum-weight realization.


Intuitively, the primary objective of introducing weight into CGMs is to
effectively represent the \new{preferences} over goals. 
%
\ignoreinshort{%%%%% gia' detto
Unlike mandatory requirements, which must be achieved in all
realizations and as such are part of user assertions inside $\Psi$, \new{optional}
(or "nice to have") requirements are goals that we would like to
include in our realization, but not compulsorily. 
}
%
The optional requirements are given rewards proportional to their
level of "preferences".  Similarly, some leaf elements can be more
expensive (in terms of effort, money, time, ...) of some others, so
that we can give them a higher penalty in order to establish our
preference.

\ignoreinshort{
\begin{example}
  \MCTODO{insert related part of example here}

%
Let us consider an example of adding weights to the goal models:

We give the requirements the following rewards:
~\REQ{Low Cost}: 100,
~\REQ{Schedule Meeting}: is mandatory,
~\REQ{Fast Schedule}: 75,
~\REQ{Good Quality Schedule}: 80, and
~\REQ{Minimal Effort}: 65.
We also give the tasks the following penalties:
~\REQ{Characterise Meeting}: 15,
~\REQ{Call Participants}: 30,
~\REQ{Email Participants}: 15,
~\REQ{Collect From System Calendar}: 5,
~\REQ{Call Partner Institutions}: 30,
~\REQ{Call Hotels And Convention Centers}: 30,
~\REQ{Get Room Suggestions}: 15,
~\REQ{List Available Rooms}: 20,
~\REQ{Use Available Room}: 10,
~\REQ{Cancel Less Important Meeting}: 40,
~\REQ{Schedule Manually}: 50,
~\REQ{Schedule Automatically}: 15,
~\REQ{Confirm Occurrence}: 5,
~\REQ{Cancel Meeting}: 5,
~\REQ{Collection Effort}: 30,
~\REQ{Matching Effort}: 30,
~\REQ{Good Participation}: 35, and
~\REQ{Minimal Conflict}: 20.
Domain assumptions can also have penalties:
~\REQ{Participants Use System Calendar}: 70 and
~\REQ{Local Room Available}: 15.

As a result, the previous realization $\mu$ (in example ~\ref{ex:CGMrealization}) has the weight  (penalties - rewards) of $(215 - 255 = -40)$ (we omit the weight of ~\REQ{Schedule Meeting} since it is the mandatory requirement). In the case of the realization:

$\mu' = \{$ ~\REQ{Low Cost}, ~\REQ{Schedule Meeting}, ~\REQ{Fast Schedule}, ~\REQ{Characterise Meeting}, ~\REQ{Collect Timetables}, ~\REQ{Find Suitable Room}, ~\REQ{Choose Schedule}, ~\REQ{Manage Meeting}, ~\REQ{By System}, ~\REQ{Call Partner Institutions}, ~\REQ{Schedule Automatically}, ~\REQ{Confirm Occurrence}, ~\REQ{Collect From System Calendar}, ~\REQ{Participants Use System Calendar}, \REQ{Good Quality Schedule}, ~\REQ{Good Participation}, ~\REQ{Minimal Conflict}, ~\REQ{Minimal Effort}, ~\REQ{Collection Effort}, ~\REQ{Matching Effort}, $R_1, R_2, R_3, R_7, R_8, R_{13}, R_{19}, R_{20}\}$

the weight of this realization is $(255 - 320 = -65)$. Clearly, $\mu'$ is better than $\mu$s since it has better reward-penalty value.
%
\end{example}
}
  


Notice that one can obtain reasonable
compromises between rewards and penalties. For instance, if the user thinks that achieving 
 an optional requirement $G_1$ is worth the effort of performing one
of tasks $G_2$ and $G_3$ but not both, then he/she can set the relative penalties
and rewards s.t.
$max(penalty(G_2),penalty(G_3))\le reward(G_1) < penalty(G_2)+penalty(G_3)$.
%
Notice also that it is possible to prioritize rewards over penalties, or
vice versa.
For instance, one may want to find a maximum-reward realization and,
if more than one can be found, choose the one of minimum penalty.
%
This can be done by assigning to the rewards of requirements values
which are 
much bigger than those assigned to the penalties of leaf
elements.~%
\footnote{E.g., it suffices to set the granularity of award values
  $10^k$ times bigger than that
 of penalty values, s.t. $k > \lceil log_{10}(N\cdot \delta)\rceil$, 
where N is the number of leaf elements and $\delta$ is their maximum
penalty value. This can be computed automatically.}
%
In general, it is possible to assign automatically
weights to optional goals by using ad hoc  algorithms. 



% \ignore{%%%%%%%%%%%%%% ENCODING COME MAX_SMT
% \begin{definition}[MaxSMT Encoding of a WCGM]
% \label{def:encoding_weighted}
% Let $\calm\defas\tuple{\calb,\cald,\Psi,\calm}$ be a WCGM.
% %
% The \new{MaxSMT encoding} of \calm is given by the pair 
% \tuple{\enc{},\cals}, where 
% $\enc{}$ is a propositional formula as in Definition~\ref{def:encoding}, 
% and \cals is a set of weighted unit clauses 
% \begin{eqnarray}
%   \cals &\defas &
% \{\ \tuple{(E_i),-\calw(E_i)}\ |\ \calw(E_i)\le 0 \}  \ \ \ \ ;root\ goals\\
% &\cup& 
% \{\ \tuple{(\neg E_i),\calw(E_i)}\ |\ \calw(E_i)\ge 0\}. \ \   \ \ ;leaf\ goals
% \end{eqnarray}
% \end{definition}

% The following fact is a straightforward consequence of Definitions
% ~\ref{def:weight} and \ref{def:encoding_weighted}.  
 
% \begin{proposition}
% \label{prop:main_weighted}
% Let $\calm\defas\tuple{\calb,\cald,\Psi,\calm}$ be a WCGM and
% $\tuple{\enc{},\cals}$ its MaxSMT encoding, let $\calt$ be a subset of its requirements,
% and let $\mu$ be a truth assignment to the variables in \calb. Then
% $\mu$ is a minimum-weight realization of \tuple{\calm,\calt} 
% if and only if
% $\mu$ is a solution to the MaxSAT problem 
% $\tuple{(\enc{} \wedge \bigwedge_{E_i\in\calt}E_i),\cals}$.
% \end{proposition}

% } %%%%%%%%% END ENCODING IN MAX-SMT





